UCB Momentum Q-learning: Correcting the bias without forgetting

We propose UCBMQ, Upper Confidence Bound Momentum Q-learning, a new algorithm for reinforcement learning in tabular and possibly stage-dependent, episodic Markov decision process. UCBMQ is based on Q-learning where we add a momentum term and rely on the principle of optimism in face of uncertainty to deal with exploration. Our new technical ingredient of UCBMQ is the use of momentum to correct the bias that Q-learning suffers while, at the same time, limiting the impact it has on the second-order term of the regret. For UCBMQ, we are able to guarantee a regret of at most $O(\sqrt{H^3SAT}+ H^4 S A )$ where $H$ is the length of an episode, $S$ the number of states, $A$ the number of actions, $T$ the number of episodes and ignoring terms in poly-$\log(SAHT)$. Notably, UCBMQ is the first algorithm that simultaneously matches the lower bound of $\Omega(\sqrt{H^3SAT})$ for large enough $T$ and has a second-order term (with respect to the horizon $T$) that scales only linearly with the number of states $S$.

==> main/algorithm.tex <==
% !TEX root = ../UCBMQ.tex
\section{\texorpdfstring{\OurAlgorithm}{} algorithm}
\label{sec:algorithm}
\subsection{Intuition}
If the agent knows the transition probabilities, it could perform real-time Q-value iteration and obtains a bounded regret (see~\citealt{efroni2019tight}). In this case upper bounds on the Q-value functions are updated as follows\footnote{We index the quantities by $n$ in this section where $n$ is the number of times the state-action pair $(s,a)$ is visited. In particular this is different from the time $t$ since, in our setting, all the state-action pair are not visited at each episode. See Section~\ref{alg:OurAlgorithm} for precise notation.}
\begin{align}
    \uQ_h^n(s,a) &= (r_h + p_h \uV_h^{n-1})(s,a) \label{eq:real_time_Q_iteration}\,.
\end{align}
When the model is unknown we can approximate it by averaging successive sample updates as in Q-learning~\citep{watkins1992q},
{\small
\begin{align}
    Q_h^n(s,a) &= \alpha_n(r_h + p_h^n \uV_h^{n-1})(s,a)+ \big(1-\alpha_n\big)Q_h^{n-1}(s,a)\,.
\end{align}
}
A usual choice for the learning rate is to set $\alpha_n = 1/n$ instead of $\alpha_n=1$ used for real-time Q-value iteration above. Unfolding the previous inequality and using Azuma–Hoeffding inequality to move for the sample expectation $p_h^i$ to the true expectation $p_h$ we have with high probability
\begin{align}
    Q_h^n &\approx r_h(s,a) + \frac{1}{n} \sum_{i=1}^{n} p_h^i \uV_{h+1}^{i-1}(s,a)\nonumber\\
    &\approx r_h(s,a)+ p_h\!\!\!\!\!\!\!\underbrace{\left(\frac{1}{n} \sum_{i=1}^{n} \uV_{h+1}^{i-1}\right)}_{:=V_{h,s,a}^n\text{ bias value function}}\!\!\!\!\!\!(s,a)\pm\!\!\!\!\! \underbrace{\sqrt{ \frac{H^2}{n}}}_{\text{variance term}} \label{eq:1_over_N_sum}\,,
\end{align}
\todoOm{Is the ``bias value function'' \textbf{only} bias? It is more like a biased upper bound, no? Maybe replace it by ``biased value function''?}
\todoPi{No it is the bias with respect to the randomness of the $p_h^i$, is it better now?}
where the bias value function of state-action $(s,a)$ encodes the bias of the estimate $Q_h^n$ with respect to the randomness of the $(p_h^i)_{i\geq 1}$. Thus choosing bonuses of order $\beta^n(s,a) \approx \sqrt{H^2/n}$ we can build upper-bound on the optimal Q-value and the value functions
\begin{align*}
  \uQ_h^n(s,a) &= Q_h^n(s,a) +\beta_h^n(s,a)\,,\\
  \uV_h^n(s) &= \max_{a\in\cA}\uQ_h^n(s,a)\,.
\end{align*}
But the bias term in~\eqref{eq:1_over_N_sum} is too large because of the too old (and potentially too large) upper-bound $\uV_{h+1}^i$ that appears in the bias value function $V_{h,s,a}^n$. Note that on contrary when the model is known (i.e. using \eqref{eq:real_time_Q_iteration}) we have $V_{h,s,a}^n = \uV_{h+1}^{n-1}$. Indeed we can only prove a regret bound exponential in the horizon $H$ in this case. \todoOm{Reference for upper bound that is exponential in $H$? Maybe \citet{jin2018is}}
\todoPi{even \citet{jin2018is} is a bit evasive about this maybe we should explain this in the appendix}

To overcome this issue \citet{jin2018is} propose to choose a learning rate of order $\alpha_n \approx H/n$ to keep only the recent upper-bounds $\uV_{h+1}^i$ in the bias value value function. Indeed in this case we have
\begin{align}
    Q_h^n(s,a) &\approx r_h(s,a)+ \frac{H}{n}\sum_{i \geq n/H}^n p_h^i \uV_{h+1}^{i-1}(s,a)\nonumber\\
    &\approx r_h(s,a)+ p_h\!\!\! \underbrace{\left(\!\!\frac{H}{n} \sum_{i\geq n/H}^n \uV_{h+1}^{n-1}\right)}_{:=V_{h,s,a}^n\text{bias value function}}\!\!(s,a) \pm \!\!\!\!\!\underbrace{\sqrt{\frac{H^3}{n}}}_{\text{variance term}}\!\!.
\label{eq:H_over_N_sum}
\end{align}
Because of the aggressive learning rate of order $H/n$ there are only $n/H$ samples in the sum of \eqref{eq:H_over_N_sum} leading to a high variance. Thus we need to add an extra $H$ factor in the bonus which leads to the sub-optimal regret bound of order $\widetilde{O}(\sqrt{H^4 S A T})$.
One workaround for this issue is to learn a reference value function, see~\citealt{zhang2020almost}, but it is not clear how to obtain a second order term that only linearly depends on the size of the state space with this approach.

We consider another approach in this paper. Following the work by~\citet{ghavamzadeh2011speedy}, we add a momentum term in the update of the Q-value that corrects the bias at the price of a small vanishing increase of the variance. Precisely for a momentum rate $\gamma_n$, we now consider the following update,
\begin{align*}
    Q_h^n(s,a) &= \alpha_n (r_h + p_h^n \uV_{h+1}^{n-1})(s,a)+ (1-\alpha_n)Q_h^{n-1}(s,a)\\
    &\quad+ \gamma_n p_h^n(\uV_{h+1}^{n-1}-V_{h,s,a}^{n-1})(s,a)\,,\\
\end{align*}
where we call $V_{h,s,a}^{n-1}$ the bias value function of state-action $(s,a)$ defined by
\begin{align*}
    V_{h,s,a}^n(s') &= (\alpha_n+\gamma_n) \uV_{h+1}^{n-1}(s')+(1-\alpha_n-\gamma_n)V_{h,s,a}^{n-1}(s')\,.
\end{align*}
Note there is a prior a different bias value function for each state-action pairs. In particular if we force the sequence of upper bounds on the value functions to be non-increasing it holds that $V_{h,s,a}^n-\uV_{h+1}^n \geq 0$.
We choose $\alpha_n \approx 1/n$ to not forget samples as in~\eqref{eq:H_over_N_sum}. The momentum rate is $\gamma_n\approx H/n$ to correct the bias that will appear otherwise as in~\eqref{eq:1_over_N_sum}.
 As explained by \citet{ghavamzadeh2011speedy}, this aggressive momentum will be compensated by the fact that $\uV_{h+1}^{n-1}-V_{h,s,a}^{n-1}$ will be small when the two quantities will converge toward $\Vstar_{h+1}$. Thanks to these choices the bias value function is the same as in \eqref{eq:H_over_N_sum}
\begin{align*}
   V_{h,s,a}^n(s') &\approx \frac{H+1}{n}(V_{h,s,a}^{n-1}-\uV_h^{n-1})(s') + \uV_h^{n-1}(s') \\
   &\approx r_h(s,a)+ \frac{H}{n} \sum_{i\geq n/H}^n  \uV_{h+1}^{i-1}(s')\,.
\end{align*}
And we have with high probability
{\small
\begin{align*}
    Q_h^n(s,a) &\approx r_h(s,a) +\frac{1}{n}\sum_{i=1}^n p_h^i\left( (H+1)\uV_{h+1}^{i-1}-V_{s,a,h}^{i-1}\right)(s,a)\\ %\label{eq:H_over_N_sum}
    &\approx r_h(s,a) + p_h\!\!\! \underbrace{\left(\frac{H}{n} \sum_{i\geq n/H}^n \uV_h^{i-1}\right)}_{\approx V_{h,s,a}^n\text{ bias value function}} \!\!
    (s,a) \pm \!\!\!\underbrace{\sqrt{ \frac{H^2}{n}}}_{\text{variance term}}\\
    &\quad\pm\underbrace{\sqrt{\frac{H^3}{n} \sum_{i=1}^n p_h(V_{h,s,a}^{n-1} - \uV_h^{n-1})(s,a)\frac{1}{n}}}_{\text{momentum variance term}}\,.
\end{align*}
}%
We thus manage to get the advantages of the two learning rates: use all the samples for the concentration and get a bias value function that only relies on the recent upper-bounds on the optimal value function. This comes only at the cost of a second variance term that will only influence the dependence on $H$ of the second order term in the regret. Note that here, for sake of simplicity, we used Hoeffding inequality which leads to a sub-optimal dependence on the horizon. That is why in the sequel we will rather use Bernstein inequality (and adapted bonuses) to obtain the optimal dependence at the first order.



% If the agent knows the transition probabilities, it could perform real-time Q-value iteration and obtains a bounded regret (see~\citealt{efroni2019tight}). In this case upper bounds on the Q-value functions are updated as follows
% \begin{align}
%     \uQ_h^t(s,a) &= \chi_h^t(s,a) \big(r_h(s,a) + p_h \uV_h^{t-1}(s,a)\big)\nonumber\\
%     &\quad+ \big(1-\chi_h^t(s,a)\big)\uQ_h^{t-1}(s,a)\,.
% \label{eq:real_time_Q_iteration}
% \end{align}
% When the model is unknown we can approximate it by averaging successive sample updates as in Q-learning~\citep{watkins1992q},
% \begin{align}
%     Q_h^t(s,a) &= \alpha_h^t(s,a) \big(r_h(s,a) + p_h^t \uV_h^{t-1}(s,a)\big)\nonumber\\
%     &\quad+ \big(1-\alpha_h^t(s,a)\big)Q_h^{t-1}(s,a)\,.
% \end{align}
% A usual choice for the learning rate is of order $\alpha_h^t(s,a) \approx \frac{1}{n_h^t(s,a)}\chi_h^t(s,a)$ instead of $\chi_h^t(s,a)=\chi_h^t(s,a)$\todoX{?} used for real-time Q-value iteration. Unfolding the previous inequality and using Hoeffding inequality we have with high probability
% \todoOm{Detail that we use Hoeffding to go from estimated $p$ to true $p$}
% \begin{align}
%     Q_h^t(s,a) &\approx \frac{1}{ n_h^k(s,a)} \sum_{k=1}^{n_h^t(s,a)} \chi_h^k(s,a)p_h^k \uV_{h+1}^{k-1}(s,a) + r_h(s,a)\nonumber\\
%     &\approx p_h\left(\underbrace{\frac{1}{ n_h^k(s,a)} \sum_{k=1}^{n_h^t(s,a)} \chi_h^k(s,a) \uV_{h+1}^{k-1}}_{:=V_{h,s,a}^t\text{ bias value function}}\right)(s,a)\nonumber\\
%     &\quad\pm \underbrace{\sqrt{H^2 \frac{1}{n_h^t(s,a)}}}_{\text{variance term}}+r_h(s,a) \label{eq:1_over_N_sum}\,,
% \end{align}
% \todoOm{Is the ``bias value function'' \textbf{only} bias? It is more like a biased upper bound, no? Maybe replace it by ``biased value function''?}
% where the bias value function of state-action $(s,a)$ encodes the bias of the estimate of the optimal Q-value function at episode $t$. Thus choosing bonuses of order $\beta_h^t(s,a) \approx \sqrt{H^2/n_h^t(s,a)}$ we can build upper-bound on the Q-value and the value functions
% \[
% \uQ_h^t(s,a) = Q_h^t(s,a) +\beta_h^t(s,a)\,,
% \]
% \[
% \uV_h^t(s) = \max_{a\in\cA}\uQ_h^t(s,a)\,.
% \]
% But the bias term in~\eqref{eq:1_over_N_sum} is too large because of the too old (and potentially too large) upper-bound $\uV_{h+1}^k$ that appears in the bias value function $V_{h,s,a}^t$. Note that on contrary when the model is known (i.e. using \eqref{eq:real_time_Q_iteration}) we have $V_{h,s,a}^t = \uV_{h+1}^{t-1}$. Indeed we can only prove a regret bound exponential in the horizon $H$ in this case. Note that this rate (babla asymptotic convergence stochastic approximation).
%
% \todoOm{Reference for upper bound that is exponential in $H$? Maybe \citet{jin2018is}}
%
% To overcome this issue \citet{jin2018is} propose to choose a learning rate of order $\alpha_h^t(s,a) \approx \frac{H}{n_h^t(s,a)}\chi_h^t(s,a)$ to keep only the recent upper-bounds $\uV_{h+1}^k$ in the bias value value function. Indeed in this case we have
% \begin{align}
%     &Q_h^t(s,a)\nonumber\\
%     &\approx \frac{H}{ n_h^t(s,a)}\sum_{k:\ n_h^k(s,a)/ n_h^t(s,a)\geq 1-1/H} \chi_h^k(s,a) p_h^k \uV_{h+1}^{k-1}(s,a)\nonumber\\
%     &\quad+ r_h(s,a)\nonumber\\
%     &\approx p_h\left( \underbrace{\frac{H}{ n_h^k(s,a)} \sum_{k:\ n_h^k(s,a)/ n_h^t(s,a)\geq 1-1/H} \chi_h^k(s,a)  \uV_{h+1}^{k-1}}_{:=V_{h,s,a}^t\text{bias value function}}\right)(s,a)\nonumber\\
%     &\quad\pm \underbrace{\sqrt{H^2 \frac{H}{n_h^t(s,a)}}}_{\text{variance term}} + r_h(s,a)\,.
% \label{eq:H_over_N_sum}
% \end{align}
% Because of the aggressive learning rate in $H/n_h^t(s,a)$ there are only $n_h^t(s,a)/H$ samples in the sum of \eqref{eq:H_over_N_sum} leading to a high variance. Thus we need to add an extra $H$ factor in the bonus which leads to the sub-optimal regret bound of order $\widetilde{O}(H\sqrt{H^3 S A T})$.
% One workaround for this issue is to learn a reference value function (see~\citealt{zhang2020almost}), but it is not clear how to obtain a second order term that only linearly depends on the size of the state space with this approach.
%
% We consider another approach in this paper. Following the work by~\citet{ghavamzadeh2011speedy}, we add a momentum term in the update of the Q-value that corrects the bias at the price of a small vanishing increase of the variance. Precisely for a momentum rate $\gamma_h^t(s,a)$, we now consider the following update,
% \begin{align*}
%     Q_h^t(s,a) &= \alpha_h^t(s,a) \big(r_h(s,a) + p_h^t \uV_{h+1}^{t-1}(s,a)\big) \\
%     &\quad+ \gamma_h^t(s,a) p_h^t(\uV_{h+1}^{t-1}-V_{h,s,a}^{t-1})(s,a)\\
%     &\quad+ \big(1-\alpha_h^t(s,a)\big)Q_h^{t-1}(s,a)\,,
% \end{align*}
% where we call $V_{h,s,a}^{t-1}$ the bias value function of state-action $(s,a)$ defined by
% \begin{align*}
%     V_{h,s,a}^t(s') &= \big(\alpha_h^t(s,a)+\gamma_h^t(s,a)\big) \uV_{h+1}^{t-1}(s')\\ &\quad+\big(1-\alpha_h^t(s,a)-\gamma_h^t(s,a)\big)V_{h,s,a}^{t-1}(s')\,.
% \end{align*}
% In particular if we force the sequence of upper bounds on the value functions to be non-increasing it holds that $V_{h,s,a}^t-\uV_{h+1}^t \geq 0$.
% We choose $\alpha_h^t(s,a) \approx \frac{1}{n_h^t(s,a)}\chi_h^t(s,a)$ to not forget samples as in~\eqref{eq:H_over_N_sum}.  The momentum rate is $\gamma_h^t(s,a)\approx \frac{H}{n_h^t(s,a)}\chi_h^t(s,a)$ to correct the bias that will appear otherwise as in~\eqref{eq:1_over_N_sum}. As explained by \citet{ghavamzadeh2011speedy}, this aggressive momentum will be compensated by the fact that $\uV_{h+1}^{t-1}-V_{h,s,a}^{t-1}$ will be small when the two quantities will converge toward $\Vstar_{h+1}$. Thanks to these choices the bias value function is the same as in \eqref{eq:H_over_N_sum}
% \begin{align*}
%    V_{h,s,a}^t(s') &\approx \frac{H+1}{n_h^t(s,a)}(V_{h,s,a}^{t-1}-\uV_h^{t-1})(s') + \uV_h^{t-1}(s') \\
%    &\approx \frac{H}{ n_h^k(s,a)} \sum_{k:\ n_h^k(s,a)/ n_h^t(s,a)\geq 1-1/H} \chi_h^k(s,a)  \uV_{h+1}^{k-1}(s')\\
%    &\quad+ r_h(s,a)\,.
% \end{align*}
% And we have with high probability
% \begin{align*}
%     Q_h^t(s,a) &\approx \frac{1}{ n_h^t(s,a)}\sum_{k} \chi_h^k(s,a) p_h^k\left( (H+1)\uV_{h+1}^{k-1}-V_{s,a,h}^{k-1}\right)(s,a)\\ %\label{eq:H_over_N_sum}
%     &\quad+ r_h(s,a)\\
%     &\approx p_h \left(\underbrace{\frac{H}{ n_h^k(s,a)} \sum_{k:\ n_h^k(s,a)/ n_h^t(s,a)\geq 1-1/H} \chi_h^k(s,a)  p_h\uV_h^{k-1}}_{\approx V_{h,s,a}^t\text{ bias value function}}\right)(s,a) \pm \underbrace{\sqrt{H^2 \frac{1}{n_h^t(s,a)}}}_{\text{variance term}}\\
%     &\quad\pm\underbrace{\sqrt{\frac{H^3}{n_h^t(s,a)} \sum_{k=1}^t p_h(V_{h,s,a}^{k-1} - \uV_h^{k-1})(s,a)\frac{1}{n_h^t(s,a)}}}_{\text{momentum variance term}}\,.
% \end{align*}
% We thus manage to get the advantages of the two learning rates: use all the samples for the concentration and get a bias value function that only relies on the recent upper-bounds on the optimal value function. This comes only at the cost of a second variance term that will only influence the dependence on $H$ of the second order term in the regret. Note that here, for sake of simplicity, we used Hoeffding inequality which leads to a sub-optimal dependence on the horizon. That is why in the sequel we will rather use Bernstein inequality (and adapted bonuses) to obtain the optimal dependence at the first order.
\subsection{Algorithm}
We initialize initial value function $V_h^0(s) = H$ for all $(s,h)\in\cS\times[H]$. We fix a learning rate $\alpha_h^t(s,a)\geq 0$ a momentum $\gamma_h^t(s,a) \geq 0$ such that $\alpha_h^t(s,a)+\gamma_h^t(s,a)\leq 1$. We also consider a bonus function $\beta_h^t(s,a)$. The update of the Q-value for \OurAlgorithm is defined as follows. We update a (biased) estimator of the optimal Q-value function as follow,
\begin{align}
    Q_h^t(s,a) &= \alpha_h^t(s,a) \big(r_h(s,a) + p_h^t \uV_{h+1}^{t-1}(s,a)\big)\nonumber\\&\quad+\gamma_h^t(s,a) p_h^t(\uV_{h+1}^{t-1}-V_{h,s,a}^{t-1})(s,a)\nonumber\\
    &\quad+ \big(1-\alpha_h^t(s,a)\big)Q_h^{t-1}(s,a)\,,
\label{eq:def_Q}
\end{align}
where the bias value function for state-action $(s,a)$ is defined by, $V_{h,s,a}^0(s')=H$,
\begin{align}
    V_{h,s,a}^t(s') &= \eta_h^t(s,a) \uV_{h+1}^{t-1}(s')+ \big(1-\eta_h^t(s,a)\big)V_{h,s,a}^{t-1}(s')\,,
\label{eq:def_V}
\end{align}
where we defined $\eta_h^t(s,a) = \alpha_h^t(s,a)+  \gamma_h^t(s,a)$. Then we build upper-confidence bound on the Q-value function by adding a bonus and on value function by taking the maximum of the upper-confidence bound on the Q-value function (and clipping the maximum to be lower than the trivial upper-bound $H$)
\[
\uQ_h^t(s,a) = Q_h^t(s,a) +\beta_h^t(s,a)\,,
\]
\[
\uV_h^t(s) =\clip\!\big( \max_{a\in\cA}\uQ_h^t(s,a),0,\uV_h^{t-1}(s)\big)\,,
\]
where the clipping operator is defined as $\clip(x,y,z) = \min(\max(x,y),z)$. We also fix the upper bounds of the value function at step $H+1$ to zero $\uV_{H+1}^t(s)=0$. Note that $\uQ_h^t(s,a)$ could be negative because of the momentum but it will still be an upper bound on the optimal Q-value with high probability see Lemma~\ref{lem:optimism}. We also enforce the upper bound on the value function to be non-increasing. We then pick the action greedily with respect to the upper-bounds $\uQ_h^t$. The complete procedure is described in Algorithm~\ref{alg:OurAlgorithm}. We choose (with the convention $0\times \infty =0$ and $1/0 = \infty$)
\[
\alpha_h^t(s,a) = \chi_h^t(s,a) \frac{1}{n_h^t(s,a)}\,,
\]
\[
\gamma_h^t(s,a) =   \chi_h^t(s,a) \frac{H}{H+n_h^t(s,a)}\frac{n_h^t(s,a)-1}{n_h^t(s,a)}\,,
\]
for the learning rate and the momentum. Note that in particular it holds $\eta_h^t(s,a)=  \chi_h^t(s,a) (H+1)/(H+n_h^t(s,a))$ which is the learning rate used by \citet{jin2018is}. We can unfold \eqref{eq:def_Q} to obtain explicit formulas for the estimate of the Q-value function when $n_h^t(s,a)>0$:
\begin{align}
  &Q_h^t(s,a)  = r_h(s,a) + \frac{1}{n_h^t(s,a)}\sum_{k=1}^{t} \chi_h^k(s,a)p_h^k \uV_h^{k-1}(s,a) \nonumber\\
  &+ \frac{1}{n_h^t(s,a)}\sum_{k=1}^{t} \chi_h^k(s,a) \rgamma_h^k(s,a) p_h^k (\uV_h^{k-1}-V_{h,s,a}^{k-1})(s,a)\,,
\label{eq:Q_unfold}
\end{align}
where the normalized momentum is definied as
\[
\rgamma_h^k(s,a) =  H \frac{n_h^t(s,a)-1}{n_h^t(s,a)+H} \,.
\] We use a bonus derived from the Bernstein inequality plus a correction term. Precisely if $n_h^t(s,a) = 0$ then $\beta_{h}^t(s,a)=H$ otherwise
\begin{align*}
\beta_h^t(s,a) &= 2\sqrt{W_h^t(s,a)\frac{\zeta}{n_h^t(s,a)}}+53H^3\frac{\zeta\log(T)}{n_h^t(s,a)}\\
\quad+& \frac{1}{H \log(T)  n_h^t(s,a) }\sum_{k=1}^t \chi_h^k(s,a)\rgamma_h^k(s,a)  p_h^k(V_{h,s,a}^{k-1}-\uV_{h+1}^{k-1})(s,a)
\end{align*}
where $\zeta$ is some exploration threshold that we will specify later and $W_h^t$ is a proxy for the variance term
{\small
\[
W_h^t(s,a) =\sum_{k=1}^t  \frac{\chi_h^k(s,a)}{n_h^t(s,a)}  p_h^k\! \left(\!\uV_{h+1}^{k-1} -  \sum_{l=1}^k  \frac{ \chi_h^l(s,a)}{n_h^t(s,a)}  p_h^l \uV_{h+1}^{l-1} \!\right)^2\!\!(s,a)\,.
\]
}
Note that the third term in the bonus will not compensate the momentum because the multiplicative factor in the bonus is of order $1/(\log(T) H n_h^t(s,a))$ whereas for the momentum it is of order $1$.
\begin{algorithm}[ht]
\centering
\caption{\OurAlgorithm}
\label{alg:OurAlgorithm}
\begin{algorithmic}[1]
  \STATE {\bfseries Input:} learning rate $\alpha_h^t$, momentum $\gamma_h^t$, bonus $\beta_h^t$.
   \STATE {\bfseries Initialize:}  $V_{h,s,a}^0=\uV_h^0 = H$ and $Q_h^0 =0$
      \FOR{$t \in[T]$}
      \FOR{$h \in [H]$}
        \STATE Play $a_h^t \in \argmax \uQ_h^{t-1}(s,a)$
        \STATE Observe $s_{h+1}^t\sim p_h(s_h^t,a_h^t)$
      \ENDFOR
      \STATE Update
      {\small
      \begin{align*}
      Q_h^t(s,a) &= \alpha_h^t(s,a) \big(r_h(s,a) + p_h^t \uV_{h+1}^{t-1}(s,a)  \big)\\
      &\quad+\big(1-\alpha_h^t(s,a)\big)Q_h^{t-1}(s,a)\\
      &\quad+\gamma_h^t(s,a) p_h^t(\uV_{h+1}^{t-1}-V_{h,s,a}^{t-1})(s,a)\\
      V_{h,s,a}^t(s') &= \eta_h^t(s,a) \uV_{h+1}^{t-1}(s')+\big(1-\eta_h^t(s,a)\big)V_{h,s,a}^{t-1}(s')\\
      \uQ_h^t(s,a) &= Q_h^t(s,a) +\beta_h^t(s,a)\\
      \uV_h^t(s) &= \clip\!\big(\max_{a\in\cA} \uQ_h^t(s,a), 0, \uV_h^{t-1}(s)\big)
      \end{align*}}
   \ENDFOR
\end{algorithmic}
\end{algorithm}


\paragraph{Complexity}

\paragraph{Model-free or model-based algorithm}

\paragraph{Comparison with variance reduction methods}
\citet{sidford2018variance}, \citet{zhang2020almost}

\subsection{Regret bound}
We assume in this section that $T\geq 3$ and $H\geq 1$. We fix $ \delta \in(0,1)$ and the exploration threshold
\begin{equation}
  \label{eq:def_zeta}
  \zeta =  \log\left(32e(2T+1)/\delta\right)\,.
\end{equation}
We prove in Appendix~\ref{app:optimism} the following lemma.
\begin{restatable}{lemma}{lemoptimism}
\label{lem:optimism}
On the event $\cE$ that holds with probability $1-\delta$ (see Section~\ref{app:concentration_value}) , $\forall t \in \N, \forall (s,a,h)\in\cS\times\cA\times[H]$ (also for $h = H+1$ for the value function), we have
\begin{align*}
  \uQ_h^t(s,a) \geq \Qstar_h(s,a) \quad\text{and}\quad \uV_h^t(s) \geq \Vstar_h(s)\,.
\end{align*}
\end{restatable}

We can now state the main result of the paper which is proved in Appendix~\ref{app:proof_regret_bound}.
\begin{theorem}
  \label{th:regret_UCBMQ}
  For \OurAlgorithm, with probability at least $1-\delta$
  \[
      R^T \leq    C_1(\delta,T) \sqrt{ H^3 SA  T}+   C_1(\delta,T)  H^4 S A
  \]
where $C_1(\delta,T)  = 126  e^{127}  \log(T) \sqrt{\zeta}$  and $C_2(\delta,T) = 3527 e^{127} \log(T)^2\zeta$.
\end{theorem}
Thus the regret of \OurAlgorithm is of order $\tO\big(\sqrt{H^3SAT} + SA H^4\big)$ matching the lower bound of $\tO\big(\sqrt{H^3SAT}\big)$ by  \citet{domingues2020episodic} $T$ large enough.



\subsection{Proof sketch of Theorem~\ref{th:regret_UCBMQ}}

